Multimodal Model-Agnostic Meta-Learning via Task-Aware Modulation

Model-agnostic meta-learners aim to acquire meta-learned parameters from similar tasks to adapt to novel tasks from the same distribution with few gradient updates. With the flexibility in the choice of models, those frameworks demonstrate appealing performance on a variety of domains such as few-shot image classification and reinforcement learning. However, one important limitation of such frameworks is that they seek a common initialization shared across the entire task distribution, substantially limiting the diversity of the task distributions that they are able to learn from. In this paper, we augment MAML with the capability to identify the mode of tasks sampled from a multimodal task distribution and adapt quickly through gradient updates. Specifically, we propose a multimodal MAML (MMAML) framework, which is able to modulate its meta-learned prior parameters according to the identified mode, allowing more efficient fast adaptation. We evaluate the proposed model on a diverse set of few-shot learning tasks, including regression, image classification, and reinforcement learning. The results not only demonstrate the effectiveness of our model in modulating the meta-learned prior in response to the characteristics of tasks but also show that training on a multimodal distribution can produce an improvement over unimodal training.

==> figures/classification_curve_fig.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{cccc}
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_5-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_5-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_5-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_5-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(a) 2 Modes 5-way trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_20-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_20-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_20-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/2_modes_20-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(b) 2 Modes 20-way trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_20-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_20-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_20-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_20-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(c) 3 Modes 5-way trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_5-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_5-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_5-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/3_modes_5-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(d) 3 Modes 20-way trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_20-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_20-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_20-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_20-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(e) 5 Modes 5-way trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_5-way_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_5-way_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_5-way_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/5_modes_5-way_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(f) 5 Modes 20-way trainings} \\
        
    \end{tabular}
    \caption{ \small
        Training curves of MAML and our method for few-shot image classification.
        We show the losses and classification accuracies for training and validation tasks after adaptation.
        MAML trainings are less stable, while ours curves are smoother.
    }
    \label{fig:classification_curve}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{tabular}{cccc}
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_1-shot_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_1-shot_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_1-shot_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_1-shot_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(a) 5-way 1-shot trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_5-shot_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_5-shot_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_5-shot_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_5-way_5-shot_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(b) 5-way 5-shot trainings} \\
        
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_1-shot_loss_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_1-shot_loss_after_update_meta_train.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_1-shot_accuracy_after_update_meta_val.png} &
        \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_1-shot_accuracy_after_update_meta_train.png} \\
        \multicolumn{4}{c}{(c) 20-way 1-shot trainings} \\
        
        % \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_3-shot_loss_after_update_meta_val.png} &
        % \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_3-shot_loss_after_update_meta_train.png} &
        % \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_3-shot_accuracy_after_update_meta_val.png} &
        % \includegraphics[width=.22\textwidth]{figures/classification/curve/Multi-MAML_20-way_3-shot_accuracy_after_update_meta_train.png} \\
        % \multicolumn{4}{c}{(d) 20-way 3-shot trainings} \\       

    \end{tabular}
    \caption{ \small
        Training curves of Multi-MAML for few-shot image classification.
        We show the losses and classification accuracies for training and validation tasks after adaptation.
    }
    \label{fig:classification_curve_multimaml}
\end{figure*}


==> text/macro.tex <==
\newcommand{\mytitle}{Multimodal Model-Agnostic Meta-Learning \\ via Task-Aware Modulation}

%%% command set {{{
\newcommand{\sun}[1]{{\color{blue}{\small\bf\sf [Sun: #1]}}}
\newcommand{\risto}[1]{{\color{red}{\small\bf\sf [Risto: #1]}}}
\newcommand{\hx}[1]{{\color{green}{\small\bf\sf [HX: #1]}}}
\newcommand{\joseph}[1]{{\color{cyan}{\small\bf\sf [Joseph: #1]}}}
\newcommand{\Skip}[1]{}

% comment out all comments
\iffalse
\newcommand{\sun}[1]{}
\newcommand{\risto}[1]{}
\newcommand{\hx}[1]{}
\newcommand{\joseph}[1]{}
\fi
%%% }}}

%%% macro {{{
% abbr
\newcommand{\etal}{\textit{et al}.}
\newcommand{\ie}{\textit{i}.\textit{e}.\ }
\newcommand{\eg}{\textit{e}.\textit{g}.\ }

% ref
\newcommand{\myfig}[1]{Figure \ref{#1}}
\newcommand{\mytable}[1]{Table \ref{#1}}
\newcommand{\myeq}[1]{Equation \ref{#1}}
\newcommand{\mysec}[1]{Section \ref{#1}}

% op
\newcommand{\tieconcat}{\mathbin{\mathpalette\dotieconcat\relax}}
\newcommand{\dotieconcat}[2]{% auxiliary macro, don't use it directly
  \text{\raisebox{.8ex}{$\smallfrown$}}%
}
\newcommand{\vspaceAfterSection}{\vspace{-0.5em}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

% rebuttal
\newcommand{\rebuttalsec}[1]{\vspace{-0.02em}\noindent\textbf{#1}}
%%% }}}

% footnote without number
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

==> text/table/classification_table_rebuttal.tex <==
\begin{table}
    \centering
    \small
    \caption{\small 5 modes: Omniglot, Mini-ImageNet, FC100, CUB, and Aircraft.}
    \scalebox{0.7}{
    \begin{tabular}{c|ccc}
    \toprule
    
    \textbf{Method \& Setup} & 5w1s & 5w5s & 20w1s\\
    
    \midrule
    
    MAML & 
    44.09\% & 54.41\% & 28.85\% \\

    Multi-MAML & 
    45.46\% & 55.92\% & 33.78\% \\

    \midrule
    MMAML (ours) & 
    \textbf{49.06}\% & \textbf{60.83}\% & \textbf{33.97}\% \\

    \bottomrule
    \end{tabular}
	}
    \label{table:classification_rebuttal}
\end{table}

%%% Wrap around text
% \Skip{
% \begin{wraptable}{r}{0.36\linewidth}
% \vspace{-1.2em}
% %\begin{table*}[htb]
%     \centering
%     \small
%     \caption{\small 5 modes: Omniglot, Mini-ImageNet, FC100, CUB, and Aircraft.}
%     \scalebox{0.75}{
%     \begin{tabular}{c|ccc}
%     \toprule
    
%     \textbf{Method \& Setup} & 5w1s & 5w5s & 20w1s\\
    
%     \midrule
    
%     MAML & 
%     44.09\% & 54.41\% & 28.85\% \\

%     Multi-MAML & 
%     45.46\% & 55.92\% & 33.78\% \\

%     \midrule
%     MMAML (ours) & 
%     \textbf{49.06}\% & \textbf{60.83}\% & \textbf{33.97}\% \\

%     \bottomrule
%     \end{tabular}
% 	}
%     \label{table:classification_rebuttal}
% % \end{table*}
% \vspace{-1.2em}
% \end{wraptable}
% }

==> text/table/regression_table_rebuttal.tex <==
\begin{table}
    \centering
    \small
    \caption{\small  MSE reduction in 5 modes regression.}
    \scalebox{0.9}{
    \begin{tabular}{lr} 
    \toprule
    MMAML & \textbf{5 Modes} \\
    \midrule
    {Before}     & {17.299} \\
    {\bf + Modulation} & {2.166}  \\
    {\bf + Adaptation} & {0.868} \\
    \bottomrule
    \end{tabular}}
    \label{table:regression}
\end{table}

    
%%% Wrap around text
% \Skip{
% \begin{wraptable}{r}{0.25\linewidth}
% \vspace{-1.2em}
%     \centering
%     \small
%     \caption{\small  MSE reduction in 5 modes regression.}
%     \scalebox{0.9}{
%     \begin{tabular}{lr} 
%     \toprule
%     MMAML & \textbf{5 Modes} \\
%     \midrule
%     {Before}     & {17.299} \\
%     {\bf + Modulation} & {2.166}  \\
%     {\bf + Adaptation} & {0.868} \\
%     \bottomrule
%     \end{tabular}}
%     \label{table:regression}
% \vspace{-1.2em}
% \end{wraptable}
% }
